Paper Abstract Writing through Editing Mechanism

We present a paper abstract writing system based on an attentive neural sequence-to-sequence model that can take a title as input and automatically generate an abstract. We design a novel Writing-editing Network that can attend to both the title and the previously generated abstract drafts and then iteratively revise and polish the abstract. With two series of Turing tests, where the human judges are asked to distinguish the system-generated abstracts from human-written ones, our system passes Turing tests by junior domain experts at a rate up to 30% and by non-expert at a rate up to 80%.

==> 4discussion.tex <==
\section{Discussion}
\begin{table}[!htb]
\small
\centering
    \begin{tabular}{|c|c|c|c|c|c|c|}%|p{0.4cm}<{\centering}
    \hline
     $n$    	& \bf 1     & \bf 2     &\bf 3   & \bf 4  &\bf 5  & \bf 6 \\ \hline%& \bf 0   
    METEOR  & $13.3$    & \bf14.0   & $13.6$ & $13.9$ & $13.8$ & $13.5$ \\ \hline%& $13.5$  
    ROUGE-L & \bf20.3   & $19.8$ 	 & $18.6$ & $19.2$ & $18.9$ & $18.8$ \\ \hline%& $19.2$  
\end{tabular}
\caption{Iteration comparison (\%)}
\label{iteration}
\end{table}
We trained and evaluated our editing approach with 1-6 iterations and the experimental results (Table~\ref{iteration}) showed that the second iteration produced the best results. The reason may be as follows. The attentive revision gate incorporates the knowledge from the paper title and the previous generated abstract. As the editing process iterates, the knowledge pool will diverge since in each iteration the generated abstract may introduce some irrelevant information. Empirically the second iteration achieved a good trade-off between good quality of generated abstract and relevance with topics in the title. 
